Crypto-Ransomware and Their Defenses: In-depth Behavioral Characterization, Discussion of Deployability, and New Insights

Crypto-ransomware has caused an unprecedented scope of impact in recent years with an evolving level of sophistication. An extensive range of studies have been on defending against ransomware and reviewing the efficacy of various protections. However, for practical defenses, deployability holds equal significance as detection accuracy. Therefore, in this study, we review 117 published ransomware defense works, categorize them by the level they are implemented at, and discuss the deployability. API-based solutions are easy to deploy and most existing works focus on machine learning-based classification. To provide more insights, we quantitively characterize the runtime behaviors of real-world ransomware samples. Based on our experimental findings, we present a possible future detection direction with our consistency analysis and API-contrast-based refinement. Moreover, we experimentally evaluate various commercial defenses and identify the security gaps. Our findings help the field understand the deployability of ransomware defenses and create more effective, practical solutions.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf \

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.02.  Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> sections/acknowledgment.tex <==
\section*{Acknowledgment}
The preferred spelling of the word ``acknowledgment'' in America is without 
an ``e'' after the ``g''. Avoid the stilted expression ``one of us (R. B. 
G.) thanks $\ldots$''. Instead, try ``R. B. G. thanks$\ldots$''. Put sponsor 
acknowledgments in the unnumbered footnote on the first page.

==> sections/commercial_setup.tex <==
\noindent \textbf{Decryptor.} For the ransomware samples we successfully run, we found decryptors for 6 of them on the NO MORE RANSOM website\footnote{https://www.nomoreransom.org/en/decryption-tools.html}. The 6 decryptors are specifically designed for 6 distinct families (Table \ref{tab:decryptor} in the appendix). Different decrypting tools require different information, such as uploading the ransom note or providing file pairs (i.e. both unencrypted and encrypted versions) for key cracking.

\noindent \textbf{Commercial Antivirus Software.}
We tested 8 different commercial antivirus software that provides protection against ransomware, namely Antivirus A (anonymized), Antivirus B (anonymized), Bitdefender, Malwarebytes, Kaspersky, McAfee, Norton, and 360 Total Security (Table~\ref{tab:av-version} in the appendix). We anonymized antivirus tools A and B following their user terms and conditions. All 8 antivirus software are generic for all types of malware with ransomware detection feature. We conducted three series of experiments. We first evaluated them with 20 real ransomware samples from 20 families active from 2015 to 2020 (marked in Table~\ref{tab:sha256} in the appendix). Each sample was compressed with the password ``infected’’ at the beginning. We uncompressed the sample and if the antivirus had no reaction, we then executed it. The machine was disconnected from the internet during all real ransomware execution to prevent spreading. Because 360 Total Security performed poorly in the offline setting, we added an online setting for it, in which we only uncompressed the samples without executing them. Second, we used two publicly available ransomware simulators to test more attack scenarios. RanSim\footnote{https://www.knowbe4.com/ransomware-simulator} simulates 23 ransomware attack scenarios. Quickbuck\footnote{https://github.com/NextronSystems/ransomware-simulator} simulates several typical ransomware behaviors. Lastly, we also used our own script to further test the behavioral detection because most antivirus tools block public simulators as malware, giving them no chance to execute. Our script simulates behaviors such as iterating and encrypting files, appending random or known ransomware file extensions, deleting volume shadow copies, and dropping ransom notes. Those ransomware-like behaviors can be run separately or together. The script is in Python 3.8. To mimic real ransomware, we statically link the crypto libraries used (PyAesCrypt\footnote{https://github.com/marcobellaccini/pyAesCrypt} and Cryptography\footnote{https://github.com/pyca/cryptography}) so that no external dependencies are needed. All tests were run on a Windows 7 VM with 2 CPUs and 4096 MB memory. The machine was reversed to the initial image after each test.

\noindent \textbf{Commercial Malware Scanner.} We test over 70 commercial malware scanners available on VirusTotal~\footnote{https://www.virustotal.com/gui/} using the 54 samples (Table~\ref{tab:sha256} in the appendix). All scanners are general purpose malware scanners in a black-box manner (i.e., the algorithm used is unknown). For each sample we scanned, the number of available scanners slightly varies (Table \ref{tab:scanner} in the appendix). We tested the scanners in three settings. First, we used them to scan the plain executable file (.exe). Second, we scanned the compressed file with a simple password “infected”. This password is used as a convention for sharing malware samples. Lastly, we made a compressed file with a random, complex password (i.e., DDfA3WFxcPMUsrsA) to test the scanners’ ability to detect obfuscated samples. We chose these settings because password obfuscation is a very low-cost way for the attacker to distribute malware samples.

==> sections/compare.tex <==
\section{Comparison with benign samples}
\label{sec:compare}

Following the same procedure as we analyze ransomware samples, we investigate 20 popular Windows applications in various categories to identify ransomware-specific behaviors and the ones shared between ransomware and goodware.

\noindent\textbf{Behavioral signatures and processes.} We observe several behavioral signatures that are shared between malicious and benign software, including checking foreground human activities (12 samples out of 20), checking system memory and disk size (13 samples), autorunning at system startup (8 samples), and deleting files from disk (2 samples). Although these features look suspicious, using them to block the threats could cause false positives. Modification of security settings and prevention system recovery are more specific to ransomware and rarely seen in regular applications. We make the distinctive ransomware behavioral signatures (i.e., shown more frequently in ransomware than in goodware) bold in Table \ref{tab:signature}. On the other hand, except for lsass.exe and explorer.exe, the processes used by ransomware are not frequently seen in regular software execution, including command line-related processes (e.g., cmd.exe and powershell.exe) and system backup-related processes (e.g., vssadmin.exe, WMIC.exe, bcdedit.exe, and wbadmin.exe).

\noindent\textbf{API call category and frequency during execution.} The majority of benign software makes the most API calls in the system, registry, and miscellaneous categories, varying from ransomware behavior. However, there are a few samples making a notable number of crypto- and file-related API calls. Dropbox (Figure \ref{fig:dropbox-crypto-calls}) makes over 3500 crypto-related calls per second in the first four seconds of execution, with a peak of over 5000 calls per second, which resembles the ransomware encryption behavior. The difference from ransomware is in the composition of the API calls made. As mentioned in Section \ref{sec:character}, the number of calls to the three crypto-related APIs made by AvosLocker is relatively evenly distributed. However, the vast majority of crypto-related API calls made by Dropbox is to a single API, i.e., \texttt{CryptDecodeObjectEx}. Moreover, Notepad++, TeamViewer, and Git make notable amount file-related calls, as shown in Figure \ref{fig:notepadpp-file-calls}, \ref{fig:teamviewer-file-calls}, and \ref{fig:git-file-calls}, respectively. By looking at the composition and call patterns, we can easily tell the difference between benign samples (Notepad++ and Teamviewer) and ransomware. However, Git shows a very ransomware-like pattern that uses a combination of multiple file-related calls and accesses 844 directories. Although the combination used by Git contains 10 APIs, which is a longer list than the ones used by ransomware samples, it contains APIs that ransomware commonly uses, such as \texttt{NtCreateFile} and \texttt{SetFilePointer}, and looks highly suspicious. Therefore, we should not make a death sentence to a program based on just one malicious sign, such as intensive crypto-related calls or intensive file-related calls, even if the sign looks like a strong indication of malicious activities. More comprehensive rules should be made for accurate judgment.


\noindent\textbf{Dynamic resolve of crypto DLLs and APIs.} Benign samples also dynamically resolve Windows libraries (DLLs) during execution, including crypto-related modules. Top modules include \texttt{advapi32.dll} (17 samples out of 20 dynamically load it), \texttt{cryptbase.dll} (13 samples), and \texttt{cryptsp.dll} (9 samples). While the same crypto-related modules are used, the most frequent APIs load by benign samples are different from ransomware. \texttt{advapi32} stands for Advanced Windows 32 Base API. This module also contains basic Windows API other than crypto functions. The most frequently loaded APIs from the crypto-related modules by benign samples are mostly from this module and are non-crypto-related, such as \texttt{EventRegister}. On the opposite, besides \texttt{advapi32}, top ransomware used APIs are also from modules \texttt{cryptsp} (e.g., \texttt{CryptAquireContextW} and \texttt{CryptGenRandom}) and rsaenh (e.g., \texttt{CPDeriveKey} and \texttt{CPSetKeyParam}). Lists of top benign software and ransomware loaded APIs are in Tables \ref{tab:benign-dynamic-resolve} and \ref{tab:ransomware-dynamic-resolve}. The results again show that the differences between regular and malicious software are often subtle and hidden in details. Coarsely defined rules may catch a number of benign programs and hurt the usability of defenses.


\hfill \break
\noindent\fbox{\begin{minipage}{0.96\linewidth}
\begin{center} \textbf{Takeaway:}\end{center}
$\star$\thinspace\thinspace\thinspace\thinspace Behaviors that destruct system copy or backup are firmer evidence of ransomware infection and should be more closely monitored than others for detection.

$\star$\thinspace\thinspace\thinspace\thinspace A single rule cannot define ransomware behavior. Some benign samples show ransomware-like behaviors at a high level, such as intensive file access.  Richer context and multiple aspects should be considered when evaluating the risk. Low-level profiling and finely defined rules are also needed to reduce false positives.

\end{minipage}}

==> sections/crypto-api.tex <==

We answer our \textbf{RQ1} with a quantitative characterization of run-time ransomware behaviors. We highlight file encryption behaviors, which are the core activities of ransomware. We also report other noteworthy behavioral signatures and discuss trend of evolution. 

\input{tables/basic}

To help understand the background of the 35 ransomware families, we systematically collect their information, including the year they first appeared, their public victims, encryption algorithms, infect vectors, and targeted systems (Table \ref{tab:basic}). 


30 of the 35 ransomware families use a hybrid scheme of encryption. They first encrypt the victim data using a symmetric algorithm and then further encrypt the symmetric keys using an asymmetric algorithm. After the attack, the victims pay the ransom to get the private key to recover their data. Advanced Encryption Standard (AES) is the most popular symmetric encryption algorithm, used by 22 families. Other prevalent symmetric algorithms include ChaCha and Salsa20, which are both stream ciphers. Found in 23 families, Rivest–Shamir–Adleman (RSA) is the most widely used asymmetric algorithm. Elliptic-curve Diffie–Hellman (ECDH) is another common asymmetric encryption (3 families).  If the implementation is correct, it would be computationally infeasible to break the private keys of RSA and ECDH through brute force.



\subsection{CryptoAPI and Library}
\label{sec:cryptoapi}

Through reverse engineering and execution analysis, we found that ransomware in our experiments uses existing cryptographic libraries or Windows CryptoAPI for encryption.

\noindent\textbf{Encryption libraries.} Although many ransomware statically links implementations of encryption functions, not all of them write the functions from scratch. From a leaked version of Babuk ransomware source code, we found that Babuk uses an elliptic curve implementation from a GitHub repository\footnote{https://github.com/agl/curve25519-donna}. Decompiling using Ghidra, we were able to match the function signatures of the Babuk sample with the curve25519\_donna function. Besides that, we also found that Avoslocker ransomware uses the Crypto++ library\footnote{https://www.cryptopp.com/} and LockBit uses Libsodium\footnote{https://doc.libsodium.org/} from the extracted text, implying the usage of existing crypto libraries. 

\noindent\textbf{CryptoAPI frequency.} Some ransomware samples make intensive CryptoAPI calls, in the order of thousands, during execution. We show AvosLocker as an example in Figure \ref{fig:avoslocker-crypto-calls}. It uses the API sequence \texttt{CryptAcquireContextA}, \texttt{CryptDecodeObjectEx},  \texttt{CryptEncrypt} for encryption. The number of calls to each of the three APIs is similar, adding up to around 4,000 calls per second.


\begin{figure}
    \centering
    \includegraphics[width=0.47\textwidth]{figures/lockbit_shell32_resolve_note2.png}
    \vspace{-3mm}
    \caption{Example of LockBit dynamically resolving libraries.}
    \label{fig:lockbit-shell32}
    \vspace{-3mm}
\end{figure}

\input{tables/dynamic_short}
\noindent\textbf{Dynamic resolution of Windows libraries.} From reverse engineering, we found some samples obfuscate strings and Windows library names, including crypto-related modules, and resolve them at runtime. Dynamic resolution is to load a module or an API using its address during execution. In this way, the usage of a module remains unknown until being executed. For instance, LockBit obfuscates strings into random text and only statically imports five modules, preventing critical information from being extracted easily. Each string and library name is encoded by XORing or subtracting a unique value, and is decoded individually during execution. Figure \ref{fig:lockbit-shell32} shows how LockBit decodes and loads \texttt{shell32.dll}. 28 such strings were found in the entry function of the LockBit. 21 of them turn out to be Windows 32 libraries, which are a much longer list than the imports. Four of them are crypto-related, namely \texttt{advapi32.dll}, \texttt{bcrypt.dll}, \texttt{crypt32.dll}, and \texttt{cryptbase.dll}. 


To further inspect this feature, we analyzed the execution report and found that the samples use \texttt{LdrLoadDll} and \texttt{LdrGetProcedureAddress} to dynamically load DLLs and APIs. By looking at the loaded modules, we found 7 crypto-related modules, namely \texttt{advapi32}, \texttt{cryptsp}, \texttt{cryptbase}, \texttt{bcryptimitives}, \texttt{crypt32}, \texttt{rsaenh}, and \texttt{bcrypt}. In the import table of the 54 ransomware samples, only \texttt{advapi32} and \texttt{crypt32} show, in 38 and 13 samples, respectively. However, all 7 crypto-related modules are dynamically loaded through \texttt{LdrLoadDll}, by 48, 33, 22, 19, 15, 8, and 3 samples, respectively. Other non-crypto modules that are frequently loaded by ransomware samples include \texttt{kernel32} (48 samples), \texttt{ole32} (42 samples), \texttt{rpcrt4} (39 samples), and \texttt{user32} (36 samples).


A short import table with few crypto-related APIs may put detection off guard and let the malware through. Encryption is one of the most distinctive features of ransomware. Hiding it increases their chance of escaping detection. One step further, although not observed in our analysis, the hacker could write dead code where the execution would never reach and put irrelevant APIs in the import table for distraction, hindering the efficiency of static analysis.



\noindent\textbf{Comparison between newer and older ransomware samples.} To find out if there exist any trends of evolution, we analyzed the usage of top dynamic resolved APIs in the newer sample group (samples from 2020 and after) and the older sample group (2019 and before). The numbers and percentage of changes are summarized in Table \ref{tab:dynamic-short}. Overall, the usage of dynamic resolutions has increased in recent years. The \texttt{rsaenh} module becomes 23.36\% more prevalent in newer samples. The usage of \texttt{CryptAquireContentW} and \texttt{CryptGenRandom}, which are APIs from \texttt{cryptsp}, increased by 26.67\% and 27.63\%, respectively. None of the samples before 2019 dynamically loaded the \texttt{brcyrptprimitives} module but its APIs are being used by up to 31.58\% of recent samples.


\noindent\textbf{Comparison with benign samples.} This comparison between ransomware and benign samples help identify the distinctions in run-time API usages, possibly. Benign samples also dynamically resolve Windows libraries, including crypto-related modules. Top modules include \texttt{advapi32} (33 samples out of 38 dynamically load it) and \texttt{cryptsp} (23 samples). While the same crypto-related modules are used, the most frequent APIs loaded by benign samples are different. Most top benign loaded APIs are from \texttt{advapi32}, which stands for Advanced Windows 32 Base API. This module also contains basic Windows API other than crypto functions, such as \texttt{EventRegister} (Table~\ref{tab:dynamic-short}).  


\vspace{1.5mm}
\noindent\colorbox{gray!13}{\fbox{\begin{minipage}{0.94\linewidth}
\textbf{Takeaway:} Many ransomware uses existing crypto libraries, such as Crypto++, Libsodium, and curve25519\_donna.

41 out of 54 ransomware samples dynamically resolve crypto modules they do not statically import.
\end{minipage}}}




==> sections/reference.tex <==
\section*{References}

Please number citations consecutively within brackets \cite{b1}. The 
sentence punctuation follows the bracket \cite{b2}. Refer simply to the reference 
number, as in \cite{b3}---do not use ``Ref. \cite{b3}'' or ``reference \cite{b3}'' except at 
the beginning of a sentence: ``Reference \cite{b3} was the first $\ldots$''

Number footnotes separately in superscripts. Place the actual footnote at 
the bottom of the column in which it was cited. Do not put footnotes in the 
abstract or reference list. Use letters for table footnotes.

Unless there are six authors or more give all authors' names; do not use 
``et al.''. Papers that have not been published, even if they have been 
submitted for publication, should be cited as ``unpublished'' \cite{b4}. Papers 
that have been accepted for publication should be cited as ``in press'' \cite{b5}. 
Capitalize only the first word in a paper title, except for proper nouns and 
element symbols.

For papers published in translation journals, please give the English 
citation first, followed by the original foreign-language citation \cite{b6}.

\begin{thebibliography}{00}
\bibitem{b1} G. Eason, B. Noble, and I. N. Sneddon, ``On certain integrals of Lipschitz-Hankel type involving products of Bessel functions,'' Phil. Trans. Roy. Soc. London, vol. A247, pp. 529--551, April 1955.
\bibitem{b2} J. Clerk Maxwell, A Treatise on Electricity and Magnetism, 3rd ed., vol. 2. Oxford: Clarendon, 1892, pp.68--73.
\bibitem{b3} I. S. Jacobs and C. P. Bean, ``Fine particles, thin films and exchange anisotropy,'' in Magnetism, vol. III, G. T. Rado and H. Suhl, Eds. New York: Academic, 1963, pp. 271--350.
\bibitem{b4} K. Elissa, ``Title of paper if known,'' unpublished.
\bibitem{b5} R. Nicole, ``Title of paper with only first word capitalized,'' J. Name Stand. Abbrev., in press.
\bibitem{b6} Y. Yorozu, M. Hirano, K. Oka, and Y. Tagawa, ``Electron spectroscopy studies on magneto-optical media and plastic substrate interface,'' IEEE Transl. J. Magn. Japan, vol. 2, pp. 740--741, August 1987 [Digests 9th Annual Conf. Magnetics Japan, p. 301, 1982].
\bibitem{b7} M. Young, The Technical Writer's Handbook. Mill Valley, CA: University Science, 1989.
\end{thebibliography}
\vspace{12pt}

==> tables/academic.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
\centering
\caption{Summary of detection features used by academic ransomware detection works. \faCheckCircle ~represents the usage of a feature. SSD-
Insider [59] and FlashGuard [60] are excluded from this table because they focus on data recovery instead of detection. CryptoAPI dynamic resolution refers to the behavior of resolving CryptoAPIs during execution without importing them. CryptoAPI usage or frequency refers to monitoring the usage of certain encryption-related functions or the overall call frequency. }
\vspace{-2mm}

\scriptsize \begin{tabular}{|
>{\columncolor[HTML]{EFEFEF}}l |c
>{\columncolor[HTML]{EFEFEF}}c c
>{\columncolor[HTML]{EFEFEF}}c c
>{\columncolor[HTML]{EFEFEF}}c c
>{\columncolor[HTML]{EFEFEF}}c c
>{\columncolor[HTML]{EFEFEF}}c |}
\hline
\cellcolor[HTML]{C0C0C0}                                                                                   & \multicolumn{10}{c|}{\cellcolor[HTML]{C0C0C0}\textbf{Features used for detection}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    \\ \hhline{|>{\arrayrulecolor{tgray2}}->{\arrayrulecolor{tblack}}|-|-|-|-|-|-|-|-|-|-|}  
\cellcolor[HTML]{C0C0C0}                                                                                   & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}}                                                                                        & \multicolumn{5}{c|}{\cellcolor[HTML]{C0C0C0}\textbf{File system}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                               & \multicolumn{2}{c|}{\cellcolor[HTML]{C0C0C0}\textbf{\begin{tabular}[c]{@{}c@{}}CryptoAPI\end{tabular}}}                                                                                                               & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}}                                                                                    & \cellcolor[HTML]{C0C0C0}                                                                                        \\ \hhline{|>{\arrayrulecolor{tgray2}}-|->{\arrayrulecolor{tblack}}|-|-|-|-|-|-|-|>{\arrayrulecolor{tgray2}}-|-|>{\arrayrulecolor{tblack}}} 
\multirow{-3}{*}{\cellcolor[HTML]{C0C0C0}\textbf{\begin{tabular}[c]{@{}l@{}}Academic\\ Work\end{tabular}}} & \multicolumn{1}{c|}{\multirow{-2}{*}{\cellcolor[HTML]{C0C0C0}\textbf{\begin{tabular}[c]{@{}c@{}}Hardware \\ counters\end{tabular}}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\textbf{\begin{tabular}[c]{@{}c@{}}File I/O\\ pattern\end{tabular}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\textbf{\begin{tabular}[c]{@{}c@{}}File I/O \\ frequency\end{tabular}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\textbf{\begin{tabular}[c]{@{}c@{}}File \\ extension\end{tabular}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\textbf{\begin{tabular}[c]{@{}c@{}}I/O entropy\\ check\end{tabular}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\textbf{Decoy}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\textbf{\begin{tabular}[c]{@{}c@{}}Dynamic\\ resolution\end{tabular}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}\textbf{\begin{tabular}[c]{@{}c@{}}Usage or\\ frequency\end{tabular}}} & \multicolumn{1}{c|}{\multirow{-2}{*}{\cellcolor[HTML]{C0C0C0}\textbf{\begin{tabular}[c]{@{}c@{}}API\\occurrence\end{tabular}}}} & \multirow{-2}{*}{\cellcolor[HTML]{C0C0C0}\textbf{\begin{tabular}[c]{@{}c@{}}Network\end{tabular}}} \\ \hline
Kok et al.~\cite{Kok2022}                                                                                  & \multicolumn{1}{c|}{}                                                                                                                & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                                                                    & \multicolumn{1}{c|}{}                                                                                               & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                                                                   & \multicolumn{1}{c|}{}                                                                                             & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                    & \multicolumn{1}{c|}{}                                                                                              & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                                                                      & \multicolumn{1}{c|}{\faCheckCircle}                                                                                              &                                                                                                                 \\ \hline
Almousa et al.~\cite{api-based}                                                                            & \multicolumn{1}{c|}{}                                                                                                                & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                                                                    & \multicolumn{1}{c|}{}                                                                                               & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                                                                   & \multicolumn{1}{c|}{}                                                                                             & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                    & \multicolumn{1}{c|}{}                                                                                              & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                                                                      & \multicolumn{1}{c|}{\faCheckCircle}                                                                                              &                                                                                                                 \\ \hline
Hwang et al.~\cite{Hwang2020two-stage}                                                                     & \multicolumn{1}{c|}{}                                                                                                                & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                                                                    & \multicolumn{1}{c|}{}                                                                                               & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                                                                   & \multicolumn{1}{c|}{}                                                                                             & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                    & \multicolumn{1}{c|}{}                                                                                              & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                                                                      & \multicolumn{1}{c|}{\faCheckCircle}                                                                                              &                                                                                                                 \\ \hline
UNVEIL~\cite{unveil}                                                                                       & \multicolumn{1}{c|}{}                                                                                                                & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\faCheckCircle}                                                      & \multicolumn{1}{c|}{}                                                                                               & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                                                                   & \multicolumn{1}{c|}{\faCheckCircle}                                                                               & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                    & \multicolumn{1}{c|}{}                                                                                              & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                                                                      & \multicolumn{1}{c|}{}                                                                                                            &                                                                                                                 \\ \hline
RansomSpector~\cite{ransomspector}                                                                         & \multicolumn{1}{c|}{}                                                                                                                & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\faCheckCircle}                                                      & \multicolumn{1}{c|}{}                                                                                               & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                                                                   & \multicolumn{1}{c|}{}                                                                                             & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                    & \multicolumn{1}{c|}{}                                                                                              & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                                                                      & \multicolumn{1}{c|}{}                                                                                                            & \faCheckCircle                                                                                                  \\ \hline
CryptoDrop~\cite{cryptolock}                                                                               & \multicolumn{1}{c|}{}                                                                                                                & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\faCheckCircle}                                                      & \multicolumn{1}{c|}{}                                                                                               & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\faCheckCircle}                                                     & \multicolumn{1}{c|}{\faCheckCircle}                                                                               & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                    & \multicolumn{1}{c|}{}                                                                                              & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                                                                      & \multicolumn{1}{c|}{}                                                                                                            &                                                                                                                 \\ \hline
ShieldFS~\cite{ShieldFS}                                                                                   & \multicolumn{1}{c|}{}                                                                                                                & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                                                                    & \multicolumn{1}{c|}{\faCheckCircle}                                                                                 & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\faCheckCircle}                                                     & \multicolumn{1}{c|}{\faCheckCircle}                                                                               & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                    & \multicolumn{1}{c|}{}                                                                                              & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                                                                      & \multicolumn{1}{c|}{}                                                                                                            &                                                                                                                 \\ \hline
R-Locker~\cite{r-locker}                                                                                   & \multicolumn{1}{c|}{}                                                                                                                & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                                                                    & \multicolumn{1}{c|}{}                                                                                               & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                                                                   & \multicolumn{1}{c|}{}                                                                                             & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\faCheckCircle}      & \multicolumn{1}{c|}{}                                                                                              & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                                                                      & \multicolumn{1}{c|}{}                                                                                                            &                                                                                                                 \\ \hline
RWGuard~\cite{Mehnaz2018rwguard}                                                                           & \multicolumn{1}{c|}{}                                                                                                                & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\faCheckCircle}                                                      & \multicolumn{1}{c|}{}                                                                                               & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                                                                   & \multicolumn{1}{c|}{}                                                                                             & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\faCheckCircle}      & \multicolumn{1}{c|}{}                                                                                              & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}\faCheckCircle}                                                        & \multicolumn{1}{c|}{}                                                                                                            &                                                                                                                 \\ \hline
POSSE~\cite{posse}                                                                                         & \multicolumn{1}{c|}{\faCheckCircle}                                                                                                  & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                                                                    & \multicolumn{1}{c|}{}                                                                                               & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                                                                   & \multicolumn{1}{c|}{}                                                                                             & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                    & \multicolumn{1}{c|}{}                                                                                              & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                                                                      & \multicolumn{1}{c|}{}                                                                                                            &                                                                                                                 \\ \hline
Aurangzeb et al.~\cite{hardware-profile}                                                                   & \multicolumn{1}{c|}{\faCheckCircle}                                                                                                  & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                                                                    & \multicolumn{1}{c|}{}                                                                                               & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                                                                   & \multicolumn{1}{c|}{}                                                                                             & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                    & \multicolumn{1}{c|}{}                                                                                              & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                                                                      & \multicolumn{1}{c|}{}                                                                                                            &                                                                                                                 \\ \hline
NetCoverse~\cite{Alhawi2018NetCoverse}                                                                     & \multicolumn{1}{c|}{}                                                                                                                & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                                                                    & \multicolumn{1}{c|}{}                                                                                               & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                                                                   & \multicolumn{1}{c|}{}                                                                                             & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                    & \multicolumn{1}{c|}{}                                                                                              & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                                                                      & \multicolumn{1}{c|}{}                                                                                                            & \faCheckCircle                                                                                                  \\ \hline
Almashhadani et al.~\cite{Almashhadani2019multi-classifier}                                                & \multicolumn{1}{c|}{}                                                                                                                & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                                                                    & \multicolumn{1}{c|}{}                                                                                               & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                                                                   & \multicolumn{1}{c|}{}                                                                                             & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                    & \multicolumn{1}{c|}{}                                                                                              & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                                                                      & \multicolumn{1}{c|}{}                                                                                                            & \faCheckCircle                                                                                                  \\ \hline
Cabaj et al.~\cite{Cabaj2016cryptowall}                                                                    & \multicolumn{1}{c|}{}                                                                                                                & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                                                                    & \multicolumn{1}{c|}{}                                                                                               & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                                                                   & \multicolumn{1}{c|}{}                                                                                             & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                    & \multicolumn{1}{c|}{}                                                                                              & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}}                                                                      & \multicolumn{1}{c|}{}                                                                                                            & \faCheckCircle                                                                                                  \\ \hline
\end{tabular}





\label{tab:academic}
\end{table*}

==> tables/architecture.tex <==
\begin{table*}[]
\centering
\caption{\small Packing and file type information of ransomware samples. SHA-256 column shows the first four digits of the samples SHA-256 hash. Entropy if the file entropy calculated out of 8. DiE considers a score higher than 6.5 as packed. Samples that are packed but not using a known packer possibly utilize their own obfuscation methods.}
% \begin{tabular}{ccccccccc}
% \hline\hline
% \textbf{\begin{tabular}[c]{@{}c@{}}Ransomware\\ Family\end{tabular}} & \textbf{SHA256} & \textbf{entropy} & \textbf{\begin{tabular}[c]{@{}c@{}}if\\ packed\end{tabular}} & \textbf{Mode} & \textbf{Architecture} & \textbf{Type} & \textbf{File Type} & \textbf{Known Packer} \\ \hline\hline
% Babuk                                                                & eb18            & 5.73 (71\%)      & no                                                           & 32-bit        & I386                  & GUI           & PE32               &                       \\ \hline
% Cerber                                                               & 0cd2            & 7.86 (98\%)      & yes                                                          & 32-bit        & I386                  & GUI           & PE32               &                       \\ \hline
% Hive                                                                 & 47db            & 6.06 (75\%)      & no                                                           & 64-bit        & AMD64                 & GUI           & PE64               &                       \\ \hline
% Jigsaw                                                               & 9c74            & 7.98 (99\%)      & yes                                                          & 32-bit        & I386                  & GUI           & PE32               & .NET Reactor          \\ \hline
% \multirow{2}{*}{LockBit}                                             & a2ad            & 6.68 (83\%)      & yes                                                          & 32-bit        & I386                  & GUI           & PE32               &                       \\ \cline{2-9} 
%                                                                      & Dec4            & 6.68 (83\%)      & yes                                                          & 32-bit        & I386                  & GUI           & PE32               &                       \\ \hline
% LockFile                                                             & 2a23            & 7.92 (98\%)      & yes                                                          & 64-bit        & AMD64                 & Console       & PE64               & UPX                   \\ \hline
% \multirow{3}{*}{Mespinoza}                                           & 4dc8            & 6.65 (83\%)      & yes                                                          & 32-bit        & I386                  & Console       & PE32               &                       \\ \cline{2-9} 
%                                                                      & 44f1            & 6.65 (83\%)      & yes                                                          & 32-bit        & I386                  & Console       & PE32               &                       \\ \cline{2-9} 
%                                                                      & af99            & 6.65 (83\%)      & yes                                                          & 32-bit        & I386                  & Console       & PE32               &                       \\ \hline
% \multirow{3}{*}{Phobos}                                              & 9dde            & 3.38 (42\%)      & no                                                           & 32-bit        & I386                  & GUI           & PE32               &                       \\ \cline{2-9} 
%                                                                      & 265d            & 6.97 (87\%)      & yes                                                          & 32-bit        & I386                  & GUI           & PE32               &                       \\ \cline{2-9} 
%                                                                      & 8710            & 6.70 (83\%)      & yes                                                          & 32-bit        & I386                  & GUI           & PE32               &                       \\ \hline
% \multirow{2}{*}{Ryuk}                                                & 9eb7            & 6.42 (80\%)      & yes                                                          & 32-bit        & I386                  & GUI           & PE32               &                       \\ \cline{2-9} 
%                                                                      & 40b8            & 5.11 (63\%)      & no                                                           & 32-bit        & I386                  & GUI           & PE32               &                       \\ \hline
% \multirow{2}{*}{Sodinokibi}                                          & 9b11            & 6.14 (76\%)      & no                                                           & 32-bit        & I386                  & GUI           & PE32               &                       \\ \cline{2-9} 
%                                                                      & fd16            & 6.76 (84\%)      & yes                                                          & 32-bit        & I386                  & GUI           & PE32               &                       \\ \hline
% \multirow{2}{*}{VirLock}                                             & 7a92            & 7.96 (99\%)      & yes                                                          & 32-bit        & I386                  & GUI           & PE32               &                       \\ \cline{2-9} 
%                                                                      & f4b1            & 7.94 (99\%)      & yes                                                          & 32-bit        & I386                  & GUI           & PE32               &                       \\ \hline
% WannaCry                                                             & ed01            & 8.00 (99\%)      & yes                                                          & 32-bit        & I386                  & GUI           & PE32               &                       \\ \hline
% TellYouThePass                                                       & 7697            & 6.04 (75\%)      & no                                                           & 64-bit        & AMD64                 & Console       & PE64               &                       \\ \hline
% Sugar                                                                & 1d4f            & 7.89 (98\%)      & yes                                                          & 32-bit        & I386                  & Console       & PE32               &                       \\ \hline
% Snatch                                                               & edad            & 7.89 (98\%)      & yes                                                          & 32-bit        & I386                  & Console       & PE32               & UPX                   \\ \hline
% MountLocker                                                          & 5eae            & 4.00 (50\%)      & no                                                           & 64-bit        & AMD64                 & GUI           & PE64               &                       \\ \hline
% \multirow{3}{*}{Lorenz}                                              & 1264            & 6.26 (78\%)      & no                                                           & 32-bit        & I386                  & Console       & PE32               &                       \\ \cline{2-9} 
%                                                                      & a0cc            & 6.31 (78\%)      & no                                                           & 32-bit        & I386                  & Console       & PE32               &                       \\ \cline{2-9} 
%                                                                      & edc2            & 6.27 (78\%)      & no                                                           & 32-bit        & I386                  & Console       & PE32               &                       \\ \hline
% Karma                                                                & 6c98            & 5.87 (73\%)      & no                                                           & 32-bit        & I386                  & GUI           & PE32               &                       \\ \hline
% HelloKitty                                                           & fa72            & 5.98 (26\%)      & no                                                           & 32-bit        & I386                  & GUI           & PE32               &                       \\ \hline
% \multirow{2}{*}{AvosLocker}                                          & 7188            & 6.63 (82\%)      & yes                                                          & 32-bit        & I386                  & Console       & PE32               &                       \\ \cline{2-9} 
%                                                                      & f810            & 6.63 (82\%)      & yes                                                          & 32-bit        & I386                  & Console       & PE32               &                       \\ \hline
% Alcatraz                                                             & 9185            & 6.48 (81\%)      & no                                                           & 32-bit        & I386                  & Console       & PE32               &                       \\ \hline
% Ragnarok                                                             & db8b            & 6.73 (84\%)      & yes                                                          & 32-bit        & I386                  & Console       & PE32               &                       \\ \hline
% Xorist                                                               & fb54            & 7.20 (90\%)      & yes                                                          & 32-bit        & I386                  & GUI           & PE32               &                       \\ \hline
% \multirow{2}{*}{MedusaLocker}                                        & 0abb            & 5.57 (69\%)      & no                                                           & 64-bit        & AMD64                 & GUI           & PE64               & \multicolumn{1}{l}{}  \\ \cline{2-9} 
%                                                                      & f5fb            & 5.57 (69\%)      & no                                                           & 64-bit        & AMD64                 & GUI           & PE64               & \multicolumn{1}{l}{}  \\ \hline\hline
% \end{tabular}

\begin{tabular}{ccccccccc}
\hline\hline
\textbf{\begin{tabular}[c]{@{}c@{}}Ransomware\\ Family\end{tabular}} & \textbf{SHA256} & \textbf{entropy} & \textbf{\begin{tabular}[c]{@{}c@{}}if\\ packed\end{tabular}} & \textbf{Mode} & \textbf{Architecture} & \textbf{Type} & \textbf{File Type} & \textbf{Known Packer} \\ \hline\hline
Alcatraz                                                             & 9185            & 6.48 (81\%)      & no                                                           & 32-bit        & I386                  & Console       & PE32               &                       \\ \hline
\multirow{2}{*}{AvosLocker}                                          & 7188            & 6.63 (82\%)      & yes                                                          & 32-bit        & I386                  & Console       & PE32               &                       \\ \cline{2-9} 
                                                                     & f810            & 6.63 (82\%)      & yes                                                          & 32-bit        & I386                  & Console       & PE32               &                       \\ \hline
Babuk                                                                & eb18            & 5.73 (71\%)      & no                                                           & 32-bit        & I386                  & GUI           & PE32               &                       \\ \hline
Cerber                                                               & 0cd2            & 7.86 (98\%)      & yes                                                          & 32-bit        & I386                  & GUI           & PE32               &                       \\ \hline
HelloKitty                                                           & fa72            & 5.98 (26\%)      & no                                                           & 32-bit        & I386                  & GUI           & PE32               &                       \\ \hline
Hive                                                                 & 47db            & 6.06 (75\%)      & no                                                           & 64-bit        & AMD64                 & GUI           & PE64               &                       \\ \hline
Jigsaw                                                               & 9c74            & 7.98 (99\%)      & yes                                                          & 32-bit        & I386                  & GUI           & PE32               & .NET Reactor          \\ \hline
Karma                                                                & 6c98            & 5.87 (73\%)      & no                                                           & 32-bit        & I386                  & GUI           & PE32               &                       \\ \hline
\multirow{2}{*}{LockBit}                                             & a2ad            & 6.68 (83\%)      & yes                                                          & 32-bit        & I386                  & GUI           & PE32               &                       \\ \cline{2-9} 
                                                                     & Dec4            & 6.68 (83\%)      & yes                                                          & 32-bit        & I386                  & GUI           & PE32               &                       \\ \hline
LockFile                                                             & 2a23            & 7.92 (98\%)      & yes                                                          & 64-bit        & AMD64                 & Console       & PE64               & UPX                   \\ \hline
\multirow{3}{*}{Lorenz}                                              & 1264            & 6.26 (78\%)      & no                                                           & 32-bit        & I386                  & Console       & PE32               &                       \\ \cline{2-9} 
                                                                     & a0cc            & 6.31 (78\%)      & no                                                           & 32-bit        & I386                  & Console       & PE32               &                       \\ \cline{2-9} 
                                                                     & edc2            & 6.27 (78\%)      & no                                                           & 32-bit        & I386                  & Console       & PE32               &                       \\ \hline
\multirow{2}{*}{MedusaLocker}                                        & 0abb            & 5.57 (69\%)      & no                                                           & 64-bit        & AMD64                 & GUI           & PE64               & \multicolumn{1}{l}{}  \\ \cline{2-9} 
                                                                     & f5fb            & 5.57 (69\%)      & no                                                           & 64-bit        & AMD64                 & GUI           & PE64               & \multicolumn{1}{l}{}  \\ \hline
\multirow{3}{*}{Mespinoza}                                           & 4dc8            & 6.65 (83\%)      & yes                                                          & 32-bit        & I386                  & Console       & PE32               &                       \\ \cline{2-9} 
                                                                     & 44f1            & 6.65 (83\%)      & yes                                                          & 32-bit        & I386                  & Console       & PE32               &                       \\ \cline{2-9} 
                                                                     & af99            & 6.65 (83\%)      & yes                                                          & 32-bit        & I386                  & Console       & PE32               &                       \\ \hline
MountLocker                                                          & 5eae            & 4.00 (50\%)      & no                                                           & 64-bit        & AMD64                 & GUI           & PE64               &                       \\ \hline
\multirow{3}{*}{Phobos}                                              & 9dde            & 3.38 (42\%)      & no                                                           & 32-bit        & I386                  & GUI           & PE32               &                       \\ \cline{2-9} 
                                                                     & 265d            & 6.97 (87\%)      & yes                                                          & 32-bit        & I386                  & GUI           & PE32               &                       \\ \cline{2-9} 
                                                                     & 8710            & 6.70 (83\%)      & yes                                                          & 32-bit        & I386                  & GUI           & PE32               &                       \\ \hline
Ragnarok                                                             & db8b            & 6.73 (84\%)      & yes                                                          & 32-bit        & I386                  & Console       & PE32               &                       \\ \hline
\multirow{2}{*}{Ryuk}                                                & 9eb7            & 6.42 (80\%)      & yes                                                          & 32-bit        & I386                  & GUI           & PE32               &                       \\ \cline{2-9} 
                                                                     & 40b8            & 5.11 (63\%)      & no                                                           & 32-bit        & I386                  & GUI           & PE32               &                       \\ \hline
Snatch                                                               & edad            & 7.89 (98\%)      & yes                                                          & 32-bit        & I386                  & Console       & PE32               & UPX                   \\ \hline
\multirow{2}{*}{Sodinokibi}                                          & 9b11            & 6.14 (76\%)      & no                                                           & 32-bit        & I386                  & GUI           & PE32               &                       \\ \cline{2-9} 
                                                                     & fd16            & 6.76 (84\%)      & yes                                                          & 32-bit        & I386                  & GUI           & PE32               &                       \\ \hline
Sugar                                                                & 1d4f            & 7.89 (98\%)      & yes                                                          & 32-bit        & I386                  & Console       & PE32               &                       \\ \hline
TellYouThePass                                                       & 7697            & 6.04 (75\%)      & no                                                           & 64-bit        & AMD64                 & Console       & PE64               &                       \\ \hline
\multirow{2}{*}{VirLock}                                             & 7a92            & 7.96 (99\%)      & yes                                                          & 32-bit        & I386                  & GUI           & PE32               &                       \\ \cline{2-9} 
                                                                     & f4b1            & 7.94 (99\%)      & yes                                                          & 32-bit        & I386                  & GUI           & PE32               &                       \\ \hline
WannaCry                                                             & ed01            & 8.00 (99\%)      & yes                                                          & 32-bit        & I386                  & GUI           & PE32               &                       \\ \hline
Xorist                                                               & fb54            & 7.20 (90\%)      & yes                                                          & 32-bit        & I386                  & GUI           & PE32               &                       \\ \hline\hline
\end{tabular}

\label{tab:architecture}
\end{table*}

==> tables/basic.tex <==
\begin{table*}[]
\centering

\caption{Information of ransomware families measured. Victims: public attack incidences. Empty means we did not find such a public case. \faEnvelopeO ~for phishing or spam email, \faFileCodeO ~for infected website, \faCloudDownload ~for infected cloud storage downloads, \faBug ~for software vulnerabilities, and RDP for remote desktop protocol.  \faWindows ~for Windows and \faLinux ~for Linux.}
\vspace{-3mm}
% \small \begin{tabular}{
% >{\columncolor[HTML]{EFEFEF}}c c
% >{\columncolor[HTML]{EFEFEF}}c c
% >{\columncolor[HTML]{EFEFEF}}c c
% >{\columncolor[HTML]{EFEFEF}}c }
% \hline
% \cellcolor[HTML]{C0C0C0}\textbf{Name}                                        & \cellcolor[HTML]{C0C0C0}\textbf{\begin{tabular}[c]{@{}c@{}}Year First\\ Appear\end{tabular}} & \cellcolor[HTML]{C0C0C0}\textbf{Victims}                                                                                                  & \cellcolor[HTML]{C0C0C0}\textbf{File Encryption}            & \cellcolor[HTML]{C0C0C0}\textbf{Key Encryption}            & \cellcolor[HTML]{C0C0C0}\textbf{Infect Vector}                                    & \cellcolor[HTML]{C0C0C0}\textbf{\begin{tabular}[c]{@{}c@{}}Target\\ System\end{tabular}} \\ \hline
% TeslaCrypt                                                                   & 2015                                                                                         &                                                                                                                                           & AES-256                                                     & RSA-2048                                                   & \faCloudDownload, Browser Exploit Kits                                            & \faWindows                                     \\ \hline
% 7ev3n                                                                        & 2016                                                                                         &                                                                                                                                           & \begin{tabular}[c]{@{}c@{}}Customized (R5A)\end{tabular} &                                                            & \faCloudDownload                                                                  & \faWindows                                     \\ \hline
% Alcatraz                                                                     & 2016                                                                                         &                                                                                                                                           & AES-256                                                     &                                                            & \faEnvelopeO, \faFileCodeO                                                        & \faWindows                                     \\ \hline
% Cerber                                                                       & 2016                                                                                         &                                                                                                                                           & RC4                                                         & \begin{tabular}[c]{@{}c@{}}RSA-880, RSA-2048\end{tabular} & \begin{tabular}[c]{@{}c@{}}\faEnvelopeO, \faFileCodeO, Malvertising\end{tabular} & \faWindows, \faLinux                           \\ \hline
% \begin{tabular}[c]{@{}c@{}}Dharma\\ (a.k.a. CrySiS)\end{tabular}             & 2016                                                                                         & Altus Baytown Hospital (ABH)                                                                                                              & AES-256-CBC                                                 & RSA-1024                                                   & RDP                                                                               & \faWindows                                     \\ \hline
% Jigsaw                                                                       & 2016                                                                                         &                                                                                                                                           & AES-128-CBC                                                 & RSA-1024                                                   & \faCloudDownload                                                                  & \faWindows                                     \\ \hline
% VirLock                                                                      & 2016                                                                                         &                                                                                                                                           & XOR or XOR-ROL                                              &                                                            & \faEnvelopeO, \faCloudDownload                                                    & \faWindows                                     \\ \hline
% Xorist                                                                       & 2016                                                                                         &                                                                                                                                           & XOR or TEA                                                  &                                                            & \faEnvelopeO, Malvertising                                                        & \faWindows                                     \\ \hline
% WannaCry                                                                     & 2017                                                                                         & \begin{tabular}[c]{@{}c@{}}Telefónica, TSMC, NHS hospital trusts\end{tabular}                                                         & AES-128-CBC                                                 & RSA-1024                                                   & \faBug(EternalBlue)                                                               & \faWindows                                     \\ \hline
% Sage                                                                         & 2017                                                                                         &                                                                                                                                           & ChaCha20                                                    & ECC                                                        & \faEnvelopeO                                                                      & \faWindows                                     \\ \hline
% \begin{tabular}[c]{@{}c@{}}Mespinoza\\ (a.k.a. Pysa)\end{tabular}            & 2018                                                                                         &                                                                                                                                           & AES-256                                                     & RSA-4096                                                   & \faCloudDownload, \faBug, RDP                                                     & \faWindows, \faLinux                           \\ \hline
% Ryuk                                                                         & 2018                                                                                         & Tribune Publishing                                                                                                                        & AES-256-CBC                                                 & RSA-4096                                                   & \faBug                                                                            & \faWindows                                     \\ \hline
% Snatch                                                                       & 2018                                                                                         & Volvo Cars Corporation                                                                                                                    & AES-128-OCFB                                                & RSA-2048                                                   & RDP                                                                               & \faWindows                                     \\ \hline
% LockBit                                                                      & 2019                                                                                         & Accenture                                                                                                                                 & AES-128                                                     & RSA-2048                                                   & \faEnvelopeO, \faBug, RDP                                                         & \faWindows, \faLinux                           \\ \hline
% Phobos                                                                       & 2019                                                                                         &                                                                                                                                           & AES-256-CBC                                                 & RSA-1024                                                   & \faEnvelopeO, RDP                                                                 & \faWindows                                     \\ \hline
% \begin{tabular}[c]{@{}c@{}}Sodinokibi\\ (a.k.a. REvil)\end{tabular} & 2019                                                                                         & \begin{tabular}[c]{@{}c@{}} JBS Foods, Brown-Forman\\Travelex, FujiFilm, Kaseya\end{tabular}                                             & Salsa20                                                     & ECDH                                                       & \begin{tabular}[c]{@{}c@{}}\faEnvelopeO\\ \faBug(Oracle WebLogic)\end{tabular}    & \faWindows, \faLinux                           \\ \hline
% TellYouThePass                                                               & 2019                                                                                         &                                                                                                                                           & AES-256                                                     & RSA-1024                                                   & \faEnvelopeO, \faBug                                                              & \faWindows, \faLinux                           \\ \hline
% Ragnarok                                                                     & 2019                                                                                         & \begin{tabular}[c]{@{}c@{}}Campari Group, Capcom\\ Energias de Portugal (EDP) \end{tabular}                                               & AES-256                                                     & RSA-4096                                                   & \faBug                                                                            & \faWindows                                     \\ \hline
% MedusaLocker                                                                 & 2019                                                                                         &                                                                                                                                           & AES-256                                                     & RSA-2048                                                   & \faEnvelopeO, RDP                                                                 & \faWindows                                     \\ \hline
% SunCrypt                                                                     & 2019                                                                                         &                                                                                                                                           & AES                                                         & RSA                                                        & \faEnvelopeO, \faBug                                                              & \faWindows                                     \\ \hline
% MarraCrypt                                                                   & 2020                                                                                         &                                                                                                                                           & AES-256                                                     & RSA-4096                                                   & \faEnvelopeO, \faBug                                                              & \faWindows                                     \\ \hline
% MountLocker                                                                  & 2020                                                                                         & Amey                                                                                                                                      & ChaCha20                                                    & RSA-2048                                                   & \begin{tabular}[c]{@{}c@{}}\faEnvelopeO, \faFileCodeO, Malvertising\end{tabular} & \faWindows, \faLinux                           \\ \hline
% SatanCryptor                                                                 & 2020                                                                                         &                                                                                                                                           & AES-256                                                     & RSA-2048                                                   & \faBug(EternalBlue), \faCloudDownload                                             & \faWindows                                     \\ \hline
% AvosLocker                                                                   & 2021                                                                                         &                                                                                                                                           & ChaCha20                                                    & RSA                                                        & \faEnvelopeO                                                                      & \faWindows                                     \\ \hline
% Babuk                                                                        & 2021                                                                                         & Washington DC PD                                                                                                                          & \begin{tabular}[c]{@{}c@{}}HC-128, ChaCha8\end{tabular}    & ECDH                                                       & \faEnvelopeO, \faBug, RDP                                                         & \faWindows, \faLinux                           \\ \hline
% \begin{tabular}[c]{@{}c@{}}DoejoCrypt \\ (a.k.a. DearCry)\end{tabular}       & 2021                                                                                         &                                                                                                                                           & AES-256                                                     & RSA-2048                                                   & \faBug(Micosoft Exchange)                                                         & \faWindows                                     \\ \hline
% Hive                                                                         & 2021                                                                                         & \begin{tabular}[c]{@{}c@{}}MediaMarkt, Missouri health center\\ Macquarie Health Corporation\\ Partnership HealthPlan of CA\end{tabular} & Customized                                                  & RSA-2048                                                   & \faEnvelopeO                                                                      & \faWindows                                     \\ \hline
% LockFile                                                                     & 2021                                                                                         & Microsoft                                                                                                                                 & AES-256-CBC                                                 & RSA-1024                                                   & \begin{tabular}[c]{@{}c@{}}ProxyShell, NTLM Relay\end{tabular}                   & \faWindows                                     \\ \hline
% Lorenz                                                                       & 2021                                                                                         & Canada Post                                                                                                                               & AES-128-CBC                                                 & RSA                                                        & \begin{tabular}[c]{@{}c@{}}\faEnvelopeO, \faFileCodeO, Malvertising\end{tabular} & \faWindows                                     \\ \hline
% Karma                                                                        & 2021                                                                                         & \begin{tabular}[c]{@{}c@{}}Canadian healthcare org (HCO)\end{tabular}                                                         & ChaCha20                                                    & ECC                                                        & \begin{tabular}[c]{@{}c@{}}\faEnvelopeO, \faFileCodeO,  Malvertising\end{tabular} & \faWindows, \faLinux                           \\ \hline
% HelloKitty                                                                   & 2021                                                                                         & CD Projekt RED                                                                                                                            & \begin{tabular}[c]{@{}c@{}}AES-128, AES-256\end{tabular}   & \begin{tabular}[c]{@{}c@{}}NTRU, ECDH\end{tabular}        & \faEnvelopeO, \faBug                                                              & \faWindows, \faLinux                           \\ \hline
% VoidCrypt                                                                    & 2021                                                                                         &                                                                                                                                           & AES-256                                                     & RSA                                                        & \faEnvelopeO                                                                      & \faWindows                                     \\ \hline
% BlackBasta                                                                   & 2022                                                                                         & American Dental Association (ADA)                                                                                                         & ChaCha20                                                    & RSA-4096                                                   & \faEnvelopeO, \faFileCodeO                                                        & \faWindows, \faLinux                           \\ \hline
% Sugar                                                                        & 2022                                                                                         & Walmart                                                                                                                                   & SCOP, RC4                                                   &                                                            & \faEnvelopeO, \faBug                                                              & \faWindows, \faLinux                           \\ \hline
% Venus                                                                        & 2022                                                                                         &                                                                                                                                           & AES-256                                                     & RSA-4096                                                   & RDP                                                                               & \faWindows                                     \\ \hline
% \end{tabular}

\scriptsize \begin{tabular}{
>{\columncolor[HTML]{EFEFEF}}c c
>{\columncolor[HTML]{EFEFEF}}c c
>{\columncolor[HTML]{EFEFEF}}c c
>{\columncolor[HTML]{EFEFEF}}c }
\hline
\cellcolor[HTML]{C0C0C0}\textbf{Name}                                      & \cellcolor[HTML]{C0C0C0}\textbf{\begin{tabular}[c]{@{}c@{}}Year First\\ Appeared\end{tabular}} & \cellcolor[HTML]{C0C0C0}\textbf{Victims}                                                                                                 & \cellcolor[HTML]{C0C0C0}\textbf{File Encryption} & \cellcolor[HTML]{C0C0C0}\textbf{Key Encryption} & \cellcolor[HTML]{C0C0C0}\textbf{Infect Vector}                                 & \cellcolor[HTML]{C0C0C0}\textbf{\begin{tabular}[c]{@{}c@{}}Target \\ System\end{tabular}} \\ \hline
TeslaCrypt                                                                 & 2015                                                                                         &                                                                                                                                          & AES-256                                          & RSA-2048                                        & \faCloudDownload, Browser Exploit Kits                                         & \faWindows                                                                                \\ \hline
7ev3n                                                                      & 2016                                                                                         &                                                                                                                                          & Customized (R5A)                                 &                                                 & \faCloudDownload                                                               & \faWindows                                                                                \\ \hline
Alcatraz                                                                   & 2016                                                                                         &                                                                                                                                          & AES-256                                          &                                                 & \faEnvelopeO, \faFileCodeO                                                     & \faWindows                                                                                \\ \hline
Cerber                                                                     & 2016                                                                                         &                                                                                                                                          & RC4                                              & RSA-880, RSA-2048                               & \faEnvelopeO, \faFileCodeO, Malvertising                                       & \faWindows, \faLinux                                                                      \\ \hline
Dharma (a.k.a. CrySiS)                                                     & 2016                                                                                         & Altus Baytown Hospital (ABH)                                                                                                             & AES-256-CBC                                      & RSA-1024                                        & RDP                                                                            & \faWindows                                                                                \\ \hline
Jigsaw                                                                     & 2016                                                                                         &                                                                                                                                          & AES-128-CBC                                      & RSA-1024                                        & \faCloudDownload                                                               & \faWindows                                                                                \\ \hline
VirLock                                                                    & 2016                                                                                         &                                                                                                                                          & XOR or XOR-ROL                                   &                                                 & \faEnvelopeO, \faCloudDownload                                                 & \faWindows                                                                                \\ \hline
Xorist                                                                     & 2016                                                                                         &                                                                                                                                          & XOR or TEA                                       &                                                 & \faEnvelopeO, Malvertising                                                     & \faWindows                                                                                \\ \hline
WannaCry                                                                   & 2017                                                                                         & \begin{tabular}[c]{@{}c@{}}Taiwan Semiconductor Manufacturing Co (TSMC)\\ NHS hospital trusts,  Telefónica\end{tabular}                  & AES-128-CBC                                      & RSA-1024                                        & \faBug(EternalBlue)                                                            & \faWindows                                                                                \\ \hline
Sage                                                                       & 2017                                                                                         &                                                                                                                                          & ChaCha20                                         & ECC                                             & \faEnvelopeO                                                                   & \faWindows                                                                                \\ \hline
Mespinoza (a.k.a. Pysa)                                                    & 2018                                                                                         &                                                                                                                                          & AES-256                                          & RSA-4096                                        & \faCloudDownload, \faBug, RDP                                                  & \faWindows, \faLinux                                                                      \\ \hline
Ryuk                                                                       & 2018                                                                                         & Tribune Publishing                                                                                                                       & AES-256-CBC                                      & RSA-4096                                        & \faBug                                                                         & \faWindows                                                                                \\ \hline
Snatch                                                                     & 2018                                                                                         & Volvo Cars Corporation                                                                                                                   & AES-128-OCFB                                     & RSA-2048                                        & RDP                                                                            & \faWindows                                                                                \\ \hline
LockBit                                                                    & 2019                                                                                         & Accenture                                                                                                                                & AES-128                                          & RSA-2048                                        & \faEnvelopeO, \faBug, RDP                                                      & \faWindows, \faLinux                                                                      \\ \hline
Phobos                                                                     & 2019                                                                                         &                                                                                                                                          & AES-256-CBC                                      & RSA-1024                                        & \faEnvelopeO, RDP                                                              & \faWindows                                                                                \\ \hline
\begin{tabular}[c]{@{}c@{}}Sodinokibi\\ (a.k.a. REvil, Sodin)\end{tabular} & 2019                                                                                         & \begin{tabular}[c]{@{}c@{}}Travelex, Brown-Forman\\ JBS Foods, FujiFilm, Kaseya\end{tabular}                                             & Salsa20                                          & ECDH                                            & \begin{tabular}[c]{@{}c@{}}\faEnvelopeO\\ \faBug(Oracle WebLogic)\end{tabular} & \faWindows, \faLinux                                                                      \\ \hline
TellYouThePass                                                             & 2019                                                                                         &                                                                                                                                          & AES-256                                          & RSA-1024                                        & \faEnvelopeO, \faBug                                                           & \faWindows, \faLinux                                                                      \\ \hline
Ragnarok                                                                   & 2019                                                                                         & \begin{tabular}[c]{@{}c@{}}Campari Group, Capcom, Energias de Portugal (EDP)\end{tabular}                                               & AES-256                                          & RSA-4096                                        & \faBug                                                                         & \faWindows                                                                                \\ \hline
MedusaLocker                                                               & 2019                                                                                         &                                                                                                                                          & AES-256                                          & RSA-2048                                        & \faEnvelopeO, RDP                                                              & \faWindows                                                                                \\ \hline
SunCrypt                                                                   & 2019                                                                                         &                                                                                                                                          & AES                                              & RSA                                             & \faEnvelopeO, \faBug                                                           & \faWindows                                                                                \\ \hline
MarraCrypt                                                                 & 2020                                                                                         &                                                                                                                                          & AES-256                                          & RSA-4096                                        & \faEnvelopeO, \faBug                                                           & \faWindows                                                                                \\ \hline
MountLocker                                                                & 2020                                                                                         & Amey                                                                                                                                     & ChaCha20                                         & RSA-2048                                        & \faEnvelopeO, \faFileCodeO, Malvertising                                       & \faWindows, \faLinux                                                                      \\ \hline
SatanCryptor                                                               & 2020                                                                                         &                                                                                                                                          & AES-256                                          & RSA-2048                                        & \faBug(EternalBlue), \faCloudDownload                                          & \faWindows                                                                                \\ \hline
AvosLocker                                                                 & 2021                                                                                         &                                                                                                                                          & ChaCha20                                         & RSA                                             & \faEnvelopeO                                                                   & \faWindows                                                                                \\ \hline
Babuk                                                                      & 2021                                                                                         & Washington DC PD                                                                                                                         & HC-128, ChaCha8                                  & ECDH                                            & \faEnvelopeO, \faBug, RDP                                                      & \faWindows, \faLinux                                                                      \\ \hline
DoejoCrypt (a.k.a. DearCry)                                                & 2021                                                                                         &                                                                                                                                          & AES-256                                          & RSA-2048                                        & \faBug(Micosoft Exchange)                                                      & \faWindows                                                                                \\ \hline
Hive                                                                       & 2021                                                                                         & \begin{tabular}[c]{@{}c@{}}MediaMarkt, Macquarie Health Corporation\\Missouri health center, Partnership HealthPlan of CA\end{tabular} & Customized                                       & RSA-2048                                        & \faEnvelopeO                                                                   & \faWindows                                                                                \\ \hline
LockFile                                                                   & 2021                                                                                         & Microsoft                                                                                                                                & AES-256-CBC                                      & RSA-1024                                        & ProxyShell, NTLM Relay                                                         & \faWindows                                                                                \\ \hline
Lorenz                                                                     & 2021                                                                                         & Canada Post                                                                                                                              & AES-128-CBC                                      & RSA                                             & \faEnvelopeO, \faFileCodeO, Malvertising                                       & \faWindows                                                                                \\ \hline
Karma                                                                      & 2021                                                                                         & Canadian healthcare organization (HCO)                                                                                                   & ChaCha20                                         & ECC                                             & \faEnvelopeO, \faFileCodeO, Malvertising                                       & \faWindows, \faLinux                                                                      \\ \hline
HelloKitty                                                                 & 2021                                                                                         & CD Projekt RED                                                                                                                           & AES-128, AES-256                                 & NTRU, ECDH                                      & \faEnvelopeO, \faBug                                                           & \faWindows, \faLinux                                                                      \\ \hline
VoidCrypt                                                                  & 2021                                                                                         &                                                                                                                                          & AES-256                                          & RSA                                             & \faEnvelopeO                                                                   & \faWindows                                                                                \\ \hline
BlackBasta                                                                 & 2022                                                                                         & American Dental Association (ADA)                                                                                                        & ChaCha20                                         & RSA-4096                                        & \faEnvelopeO, \faFileCodeO                                                     & \faWindows, \faLinux                                                                      \\ \hline
Sugar                                                                      & 2022                                                                                         & Walmart                                                                                                                                  & SCOP, RC4                                        &                                                 & \faEnvelopeO, \faBug                                                           & \faWindows, \faLinux                                                                      \\ \hline
Venus                                                                      & 2022                                                                                         &                                                                                                                                          & AES-256                                          & RSA-4096                                        & RDP                                                                            & \faWindows                                                                                \\ \hline
\end{tabular}

% \scriptsize\begin{tabular}{
% >{\columncolor[HTML]{EFEFEF}}c c
% >{\columncolor[HTML]{EFEFEF}}c c
% >{\columncolor[HTML]{EFEFEF}}c c
% >{\columncolor[HTML]{EFEFEF}}c }
% \hline
% \cellcolor[HTML]{C0C0C0}\textbf{Name}                                        & \cellcolor[HTML]{C0C0C0}\textbf{\begin{tabular}[c]{@{}c@{}}Year First\\ Appear\end{tabular}} & \cellcolor[HTML]{C0C0C0}\textbf{Victims}                                                                                                  & \cellcolor[HTML]{C0C0C0}\textbf{File Encryption}          & \cellcolor[HTML]{C0C0C0}\textbf{Key Encryption}            & \cellcolor[HTML]{C0C0C0}\textbf{Infect Vector}                                    & \cellcolor[HTML]{C0C0C0}\textbf{Target System} \\ \hline
% Alcatraz                                                                     & 2016                                                                                         &                                                                                                                                           & AES-256                                                   &                                                            & \faEnvelopeO, \faFileCodeO                                                        & \faWindows                                     \\ \hline
% Cerber                                                                       & 2016                                                                                         &                                                                                                                                           & RC4                                                       & \begin{tabular}[c]{@{}c@{}}RSA-880\\ RSA-2048\end{tabular} & \begin{tabular}[c]{@{}c@{}}\faEnvelopeO, \faFileCodeO, Malvertising\end{tabular} & \faWindows, \faLinux                           \\ \hline
% Jigsaw                                                                       & 2016                                                                                         &                                                                                                                                           & AES-128-CBC                                               & RSA-1024                                                   & \faCloudDownload                                                                  & \faWindows                                     \\ \hline
% VirLock                                                                      & 2016                                                                                         &                                                                                                                                           & XOR or XOR-ROL                                            &                                                            & \faEnvelopeO, \faCloudDownload                                                    & \faWindows                                     \\ \hline
% Xorist                                                                       & 2016                                                                                         &                                                                                                                                           & XOR or TEA                                                &                                                            & \faEnvelopeO, Malvertising                                                        & \faWindows                                     \\ \hline
% WannaCry                                                                     & 2017                                                                                         & \begin{tabular}[c]{@{}c@{}}TSMC, Telefónica\\ NHS hospital trusts\end{tabular}                & AES-128-CBC                                               & RSA-1024                                                   & \faBug(EternalBlue)                                                               & \faWindows                                     \\ \hline
% \begin{tabular}[c]{@{}c@{}}Mespinoza\\ (a.k.a. Pysa)\end{tabular}            & 2018                                                                                         &                                                                                                                                           & AES-256                                                   & RSA-4096                                                   & \faCloudDownload, \faBug, RDP                                                     & \faWindows, \faLinux                           \\ \hline
% Ryuk                                                                         & 2018                                                                                         & Tribune Publishing                                                                                                                        & AES-256-CBC                                               & RSA-4096                                                   & \faBug                                                                            & \faWindows                                     \\ \hline
% Snatch                                                                       & 2018                                                                                         & Volvo Cars Corporation                                                                                                                    & AES-128-OCFB                                              & RSA-2048                                                   & RDP                                                                               & \faWindows                                     \\ \hline
% LockBit                                                                      & 2019                                                                                         & Accenture                                                                                                                                 & AES-128                                                   & RSA-2048                                                   & \faEnvelopeO, \faBug, RDP                                                         & \faWindows, \faLinux                           \\ \hline
% Phobos                                                                       & 2019                                                                                         &                                                                                                                                           & AES-256-CBC                                               & RSA-1024                                                   & \faEnvelopeO, RDP                                                                 & \faWindows                                     \\ \hline
% \begin{tabular}[c]{@{}c@{}}Sodinokibi\\ (a.k.a. REvil)\end{tabular} & 2019                                                                                         & \begin{tabular}[c]{@{}c@{}}Travelex, JBS Foods, Kaseya\\ Brown-Forman, FujiFilm \end{tabular}                                           & Salsa20                                                   & ECDH                                                       & \begin{tabular}[c]{@{}c@{}}\faEnvelopeO\\ \faBug(Oracle WebLogic)\end{tabular} & \faWindows, \faLinux                           \\ \hline
% TellYouThePass                                                               & 2019                                                                                         &                                                                                                                                           & AES-256                                                   & RSA-1024                                                   & \faEnvelopeO, \faBug                                                              & \faWindows, \faLinux                           \\ \hline
% Ragnarok                                                                     & 2019                                                                                         & \begin{tabular}[c]{@{}c@{}}Campari Group, Capcom\\ Energias de Portugal (EDP) \end{tabular}                                               & AES-256                                                   & RSA-4096                                                   & \faBug                                                                            & \faWindows                                     \\ \hline
% MedusaLocker                                                                 & 2019                                                                                         &                                                                                                                                           & AES-256                                                   & RSA-2048                                                   & \faEnvelopeO, RDP                                                                 & \faWindows                                     \\ \hline
% MountLocker                                                                  & 2020                                                                                         & Amey                                                                                                                                      & ChaCha20                                                  & RSA-2048                                                   & \begin{tabular}[c]{@{}c@{}}\faEnvelopeO, \faFileCodeO, Malvertising\end{tabular} & \faWindows, \faLinux                           \\ \hline
% Babuk                                                                        & 2021                                                                                         & Washington DC PD                                                                                                                          & \begin{tabular}[c]{@{}c@{}}HC-128 or ChaCha8\end{tabular}  & ECDH                                                       & \faEnvelopeO, \faBug, RDP                                                         & \faWindows, \faLinux                           \\ \hline
% Hive                                                                         & 2021                                                                                         & \begin{tabular}[c]{@{}c@{}}MediaMarkt\\ Missouri health center\\ Macquarie Health Corporation\\ Partnership HealthPlan of CA\end{tabular} & Customized                                                & RSA-2048                                                   & \faEnvelopeO                                                                      & \faWindows                                     \\ \hline
% LockFile                                                                     & 2021                                                                                         & Microsoft                                                                                                                                 & AES-256-CBC                                               & RSA-1024                                                   & \begin{tabular}[c]{@{}c@{}}ProxyShell\\ NTLM Relay\end{tabular}                   & \faWindows                                     \\ \hline
% Lorenz                                                                       & 2021                                                                                         & Canada Post                                                                                                                               & AES-128-CBC                                               & RSA                                                        & \begin{tabular}[c]{@{}c@{}}\faEnvelopeO, \faFileCodeO, Malvertising\end{tabular} & \faWindows                                     \\ \hline
% Karma                                                                        & 2021                                                                                         & \begin{tabular}[c]{@{}c@{}}Canadian healthcare organization (HCO)\end{tabular}                                                         & ChaCha20                                                  & ECC                                                        & \begin{tabular}[c]{@{}c@{}}\faEnvelopeO, \faFileCodeO, Malvertising\end{tabular} & \faWindows, \faLinux                           \\ \hline
% HelloKitty                                                                   & 2021                                                                                         & CD Projekt RED                                                                                                                            & \begin{tabular}[c]{@{}c@{}}AES-128 or AES-256\end{tabular} & \begin{tabular}[c]{@{}c@{}}NTRU or ECDH\end{tabular}        & \faEnvelopeO, \faBug                                                              & \faWindows, \faLinux                           \\ \hline
% AvosLocker                                                                   & 2021                                                                                         &                                                                                                                                           & ChaCha20                                                  & RSA                                                        & \faEnvelopeO                                                                      & \faWindows                                     \\ \hline
% Sugar                                                                        & 2022                                                                                         & Walmart                                                                                                                                   & SCOP or RC4                                                 &                                                            & \faEnvelopeO, \faBug                                                              & \faWindows, \faLinux                           \\ \hline
% \end{tabular}




\label{tab:basic}
\end{table*}

==> tables/days.tex <==
\begin{table}[]
\centering
\caption{Days the specified ransomware stayed unknown. The SHA-256 column shows the first 4 digits of the sample hash. The days unknown represent the length between they are first seen in the wild and first submitted to ViruaTotal.}
\vspace{-1mm}
\scriptsize \begin{tabular}{
>{\columncolor[HTML]{EFEFEF}}c c
>{\columncolor[HTML]{EFEFEF}}c c
>{\columncolor[HTML]{EFEFEF}}c }
\hline
\cellcolor[HTML]{C0C0C0}\textbf{\begin{tabular}[c]{@{}c@{}}Ransomware\\ Family\end{tabular}} & \cellcolor[HTML]{C0C0C0}\textbf{\begin{tabular}[c]{@{}c@{}}SHA\\ 256\end{tabular}} & \cellcolor[HTML]{C0C0C0}\textbf{\begin{tabular}[c]{@{}c@{}}First Seen \\ in the Wild\end{tabular}} & \cellcolor[HTML]{C0C0C0}\textbf{\begin{tabular}[c]{@{}c@{}}First \\ Submission\end{tabular}} & \cellcolor[HTML]{C0C0C0}\textbf{\begin{tabular}[c]{@{}c@{}}Days \\ Unknown\end{tabular}} \\ \hline
Alcatraz                                                                                     & 9185                                    & 2016-10-05                                                                                         & 2016-10-05                                                                                   & 0                                                                                            \\ \hline
LockFile                                                                                     & 2a23                                    & 2021-04-19                                                                                         & 2021-08-24                                                                                   & 127                                                                                          \\ \hline
MedusaLocker                                                                                 & 0abb                                    & 2021-01-09                                                                                         & 2021-08-08                                                                                   & 211                                                                                          \\ \hline
Mespinoza                                                                                    & 4dc8                                    & 2021-01-05                                                                                         & 2021-01-05                                                                                   & 0                                                                                            \\ \hline
Phobos                                                                                       & 265d                                    & 2021-04-09                                                                                         & 2021-08-23                                                                                   & 136                                                                                          \\ \hline
Ryuk                                                                                         & 9eb7                                    & 2020-11-20                                                                                         & 2021-03-10                                                                                   & 110                                                                                          \\ \hline
Xorist                                                                                       & fb54                                    & 2021-01-04                                                                                         & 2021-01-04                                                                                   & 0                                                                                            \\ \hline
\end{tabular}
\label{tab:days}
% \vspace{-3mm}
\end{table}

==> tables/dynamic_resolve.tex <==
\begin{table}[]
\caption{\small Top dynamically loaded APIs from crypto-related modules by ransomware samples. Count is the number of samples that load this API during execution.}
\centering

\scriptsize\begin{tabular}{
>{\columncolor[HTML]{EFEFEF}}l c
>{\columncolor[HTML]{EFEFEF}}c }
\hline
\cellcolor[HTML]{C0C0C0}\textbf{API} & \cellcolor[HTML]{C0C0C0}\textbf{Module} & \cellcolor[HTML]{C0C0C0}\textbf{Count} \\ \hline
CryptReleaseContext                  & cryptsp                                 & 26                                     \\ \hline
RegCloseKey                          & advapi32                                & 23                                     \\ \hline
RegOpenKeyExW                        & advapi32                                & 20                                     \\ \hline
OpenProcessToken                     & advapi32                                & 19                                     \\ \hline
OpenThreadToken                      & advapi32                                & 19                                     \\ \hline
GetTokenInformation                  & advapi32                                & 19                                     \\ \hline
CryptAcquireContextW                 & cryptsp                                 & 18                                     \\ \hline
LookupAccountSidW                    & advapi32                                & 16                                     \\ \hline
RegEnumKeyW                          & advapi32                                & 15                                     \\ \hline
CryptGenRandom                       & cryptsp                                 & 15                                     \\ \hline
CreateWellKnownSid                   & advapi32                                & 15                                     \\ \hline
CPDestroyKey                         & rsaenh                                  & 13                                     \\ \hline
CPDestroyHash                        & rsaenh                                  & 13                                     \\ \hline
CPDeriveKey                          & rsaenh                                  & 13                                     \\ \hline
CPSetKeyParam                        & rsaenh                                  & 13                                     \\ \hline
CPDecrypt                            & rsaenh                                  & 13                                     \\ \hline
CPCreateHash                         & rsaenh                                  & 13                                     \\ \hline
CPSetProvParam                       & rsaenh                                  & 13                                     \\ \hline
CPDuplicateHash                      & rsaenh                                  & 13                                     \\ \hline
CPSignHash                           & rsaenh                                  & 13                                     \\ \hline
CPVerifySignature                    & rsaenh                                  & 13                                     \\ \hline
CPAcquireContext                     & rsaenh                                  & 13                                     \\ \hline
CPSetHashParam                       & rsaenh                                  & 13                                     \\ \hline
CPDuplicateKey                       & rsaenh                                  & 13                                     \\ \hline
CPGetUserKey                         & rsaenh                                  & 13                                     \\ \hline
CPGetProvParam                       & rsaenh                                  & 13                                     \\ \hline
CPHashData                           & rsaenh                                  & 13                                     \\ \hline
CPEncrypt                            & rsaenh                                  & 13                                     \\ \hline
CPImportKey                          & rsaenh                                  & 13                                     \\ \hline
CPGetKeyParam                        & rsaenh                                  & 13                                     \\ \hline
CPHashSessionKey                     & rsaenh                                  & 13                                     \\ \hline
CPGetHashParam                       & rsaenh                                  & 13                                     \\ \hline
CPGenRandom                          & rsaenh                                  & 13                                     \\ \hline
IsTextUnicode                        & advapi32                                & 13                                     \\ \hline
CPGenKey                             & rsaenh                                  & 13                                     \\ \hline
CPReleaseContext                     & rsaenh                                  & 13                                     \\ \hline
CPExportKey                          & rsaenh                                  & 13                                     \\ \hline
\end{tabular}

\label{tab:ransomware-dynamic-resolve}
\end{table}




\begin{table}[]
\caption {\small Top dynamically loaded APIs from crypto-related modulesby benign software samples. Count is the number of samples that load this API during execution.}
\centering

\scriptsize\begin{tabular}{
>{\columncolor[HTML]{EFEFEF}}l c
>{\columncolor[HTML]{EFEFEF}}c }
\hline
\cellcolor[HTML]{C0C0C0}\textbf{API} & \cellcolor[HTML]{C0C0C0}\textbf{Module} & \cellcolor[HTML]{C0C0C0}\textbf{Count} \\ \hline
EventUnregister                      & advapi32                                & 13                                     \\ \hline
EventRegister                        & advapi32                                & 13                                     \\ \hline
EventWrite                           & advapi32                                & 13                                     \\ \hline
GetTokenInformation                  & advapi32                                & 12                                     \\ \hline
OpenProcessToken                     & advapi32                                & 12                                     \\ \hline
RegisterTraceGuidsW                  & advapi32                                & 11                                     \\ \hline
OpenThreadToken                      & advapi32                                & 11                                     \\ \hline
RegEnumKeyW                          & advapi32                                & 11                                     \\ \hline
RegCloseKey                          & advapi32                                & 11                                     \\ \hline
EventEnabled                         & advapi32                                & 11                                     \\ \hline
UnregisterTraceGuids                 & advapi32                                & 10                                     \\ \hline
RegOpenKeyExW                        & advapi32                                & 10                                     \\ \hline
AllocateAndInitializeSid             & advapi32                                & 10                                     \\ \hline
GetLengthSid                         & advapi32                                & 9                                      \\ \hline
InitializeSecurityDescriptor         & advapi32                                & 9                                      \\ \hline
IsTextUnicode                        & advapi32                                & 9                                      \\ \hline
IsValidSid                           & advapi32                                & 9                                      \\ \hline
RegDeleteTreeW                       & advapi32                                & 9                                      \\ \hline
RegDeleteTreeA                       & advapi32                                & 9                                      \\ \hline
CopySid                              & advapi32                                & 9                                      \\ \hline
RegGetValueW                         & advapi32                                & 9                                      \\ \hline
AddAccessAllowedAceEx                & advapi32                                & 9                                      \\ \hline
InitializeAcl                        & advapi32                                & 9                                      \\ \hline
SetSecurityDescriptorDacl            & advapi32                                & 9                                      \\ \hline
RegQueryValueW                       & advapi32                                & 8                                      \\ \hline
RegOpenKeyW                          & advapi32                                & 8                                      \\ \hline
CryptReleaseContext                  & cryptsp                                 & 8                                      \\ \hline
% CheckTokenMembership                 & advapi32                                & 7                                      \\ \hline
% CreateWellKnownSid                   & advapi32                                & 6                                      \\ \hline
% LookupAccountSidW                    & advapi32                                & 6                                      \\ \hline
% RegDeleteKeyExW                      & advapi32                                & 6                                      \\ \hline
\end{tabular}

\label{tab:benign-dynamic-resolve}
\end{table}



==> tables/list20.tex <==
\begin{table}[]
\centering
\caption{\small The samples used for testing commercial antivirus software. SHA-256 column shows the first 4 digits of the sample. }
\begin{tabular}{ccc}
\hline\hline
\textbf{\begin{tabular}[c]{@{}c@{}}Ransomware\\ Family\end{tabular}} & \textbf{SHA-256} &  \\ \hline\hline
AvosLocker                                                           & 7188             &  \\ \hline
Babuk                                                                & eb18             &  \\ \hline
Cerber                                                               & 0cd2             &  \\ \hline
HelloKitty                                                           & fa72             &  \\ \hline
Hive                                                                 & 47db             &  \\ \hline
Jigsaw                                                               & 9c74             &  \\ \hline
Karma                                                                & 6c98             &  \\ \hline
LockBit                                                              & a2ad             &  \\ \hline
LockFile                                                             & 2a23             &  \\ \hline
Lorenz                                                               & 1264             &  \\ \hline
Mespinoza                                                            & 4dc8             &  \\ \hline
MountLocker                                                          & 5eae             &  \\ \hline
Phobos                                                               & 9dde             &  \\ \hline
Ryuk                                                                 & 9eb7             &  \\ \hline
Snatch                                                               & edad             &  \\ \hline
Sodinokibi                                                           & 9b11             &  \\ \hline
Sugar                                                                & 1d4f             &  \\ \hline
TellYouThePass                                                       & 7696             &  \\ \hline
VirLock                                                              & 7a92             &  \\ \hline
WannaCry                                                             & ed01             &  \\ \hline\hline
\end{tabular}
\label{tab:list20}
\end{table}

==> tables/scanner-short.tex <==
\begin{table}[]
\caption{The average number of alters from over 70 malware scanners on VirusTotal. The plain file column shows the results of scanning plain .exe ransomware samples. Simple pwd and complex pwd columns show the scanning results for simple password- and complex password- compressed files (in .zip format), respectively. Full results of each are shown in appendix.}
\scriptsize \begin{tabular}{ccc}
\hline
\rowcolor[HTML]{C0C0C0} 
\textbf{Plain File}        & \textbf{Simple pwd} & \textbf{Complex pwd}         \\ \hline
\cellcolor[HTML]{EFEFEF}56 & 1                   & \cellcolor[HTML]{EFEFEF}0.33 \\ \hline
\end{tabular}
\label{tab:scanner-short}

\end{table}

==> tables/stage.tex <==
\begin{table}[]
\centering

\caption{ Mean and median of ransomware execution stage duration. }
\begin{tabular}{|c|cc|}
\hline
\rowcolor[HTML]{C0C0C0} 
\cellcolor[HTML]{C0C0C0}                                 & \multicolumn{2}{c|}{\cellcolor[HTML]{C0C0C0}\textbf{Duration}}                   \\ \hhline{|>{\arrayrulecolor{gray!53}}->{\arrayrulecolor{tblack}}|-|-|}
\rowcolor[HTML]{C0C0C0} 
\multirow{-2}{*}{\cellcolor[HTML]{C0C0C0}\textbf{Stage}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}Mean} & Median                       \\ \hline
\cellcolor[HTML]{EFEFEF}Pre-encryption                   & \multicolumn{1}{c|}{21.6s}                        & \cellcolor[HTML]{EFEFEF}1.0s \\ \hline
\cellcolor[HTML]{EFEFEF}Encryption                       & \multicolumn{1}{c|}{349s}                         & \cellcolor[HTML]{EFEFEF}424s \\ \hline
\end{tabular}
\label{tab:stage}
\end{table}
